Efficient sequential and parallel algorithms for multistage stochastic integer programming using proximity

We consider the problem of solving integer programs of the form $\min \{\,c^\intercal x\ \colon\ Ax=b, x\geq 0\}$, where $A$ is a multistage stochastic matrix in the following sense: the primal treedepth of $A$ is bounded by a parameter $d$, which means that the columns of $A$ can be organized into a rooted forest of depth at most $d$ so that columns not bound by the ancestor/descendant relation in the forest do not have non-zero entries in the same row. We give an algorithm that solves this problem in fixed-parameter time $f(d,\|A\|_{\infty})\cdot n\log^{O(2^d)} n$, where $f$ is a computable function and $n$ is the number of rows of $A$. The algorithm works in the strong model, where the running time only measures unit arithmetic operations on the input numbers and does not depend on their bitlength. This is the first fpt algorithm for multistage stochastic integer programming to achieve almost linear running time in the strong sense. For the case of two-stage stochastic integer programs, our algorithm works in time $2^{(2\|A\|_\infty)^{O(r(r+s))}}\cdot n\log^{O(rs)} n$. The algorithm can be also parallelized: we give an implementation in the PRAM model that achieves running time $f(d,\|A\|_{\infty})\cdot \log^{O(2^d)} n$ using $n$ processors. The main conceptual ingredient in our algorithms is a new proximity result for multistage stochastic integer programs. We prove that if we consider an integer program $P$, say with a constraint matrix $A$, then for every optimum solution to the linear relaxation of $P$ there exists an optimum (integral) solution to $P$ that lies, in the $\ell_{\infty}$-norm, within distance bounded by a function of $\|A\|_{\infty}$ and the primal treedepth of $A$. On the way to achieve this result, we prove a generalization and considerable improvement of a structural result of Klein for multistage stochastic integer programs.

==> proximity_short.tex <==
\section{Some proximity results}\label{sec:proximity}

In this section we will give upper bound on the maximum distance of optimal fractional solutions to optimal integral solutions whenever the underlying constraint matrix $A$ is $(r,s)$ stochastic or has bounded tree-width. This is Lemma \cref{lem:proximity-multi} and \cref{lem:proximity-two} respectively. At the heart of these proximity bounds is a variant of a lemma due to Klein, we provide a proof in the last subsection.\\  
To facilitate the discussion of proximity, we introduce the following definition.

\begin{definition}
 Let $P=(x,A,b,c)$ be a linear program in the form~\eqref{eq:ilp-eq-form}. The {\em{proximity}} of~$P$, denoted $\proximity(P)$, is the infimum of reals $\rho\geq 0$ satisfying the following: for every fractional solution $x^\frc\in \sol^\R(P)$ and integral solution $x^\itg\in\sol^\Z(P)$, there is an integral solution $x^\itgo\in \sol^\Z(P)$ such that 
 \[\|x^\itgo-x^\frc\|_\infty\leq \rho
 \qquad \text{ and }\qquad x^\itgo -x^\frc \cleq x^\itg - x^\frc.\]
\end{definition}
\noindent
Geometrically, the condition $x^\itg -x^\frc \cleq x^\itgo - x^\frc$ states that $x^\itgo$ is contained in the axis parallel box spanned by $x^\frc$ and $x^\itg$, see Figure \ref{illustration:rectangle}. This notion of proximity is independent of the objective function and only depends on the underlying polyhedron $\sol^\R(P)$. However, this definition still relates the distance of optimal fractional solutions to optimal integral solutions.

\begin{lemma}\label{lem:proximity-optimal}
 Suppose $P=(x,A,b,c)$ is a linear program in the form~\eqref{eq:ilp-eq-form}. Then for every optimal fractional solution $x^\frc$ to $P$, there exists an optimal integral solution $x^\itg$ to $P$ satisfying
 $$\|x^\itg-x^\frc\|_\infty\leq \proximity(P).$$
\end{lemma}
\begin{figure}

	\centering
		\begin{tikzpicture}
		\draw[help lines, color=gray!50, dashed] (-0.3,-0.3) grid (6.9,3.4);
		\draw[->,thick] (-0.3,0)--(7,0) node[right]{};
		\draw[->,thick] (0,-0.3)--(0,3.5) node[above]{};
		\node[fill, draw, circle, inner sep=1pt, black, label={0:$x^{\star}$}] at (5.2,0.5) {};
		\node[label={0:$x \geq 0$}] at (6, 1.3){};
		\node[fill, draw, circle, inner sep=1pt, black, label={180:$x^{\diamond}$}] at (1,3) {};
		\node[fill, draw, circle, inner sep=1pt, black, label={0:$x^{\itgo}$}] at (4,2) {};
		\draw[black] (1,3) rectangle (5.2, 0.5);
		\draw[->, dashed, gray] (4,2) -- (1,3);
		\node[fill, draw, circle, inner sep=1pt, black, label={90:$x^{\bullet}$}] at (2.2,1.5) {};
		\draw[->, dashed, gray] (5.2, 0.5) -- (2.2,1.5);
	\end{tikzpicture}
\caption{$x^{\itgo} - x^{\frc} \cleq x^\frc - x^\itg$, $x^\itgo$ is in the rectangle spanned by $x^\itg$ and $x^\frc$.}	
\label{illustration:rectangle}
\end{figure}
\begin{proof}
 Let $x^\itg$ a optimal integral solution with minimal $\ell_{\infty}$ distance to $x^\frc$. Assume towards a contradiction that $\|x^\itg - x^\frc\|_\infty >\proximity(P)$. By the definition of proximity, there is an integral solution $x^\itgo$ to $P$ such that $\|x^\itgo - x^\frc\|_\infty\le\proximity(P)$ and $x^\itgo -x^\frc \cleq x^\itg - x^\frc$, see Figure \ref{illustration:rectangle} for an illustration. By optimality of $x^\itg$ we get that
 \[c^\trans (x^\itg-x^\itgo) < 0.\]
 Set $x^\frco\coloneqq x^\frc + (x^\itg-x^\itgo)$. $Ax^\frco = b$ and, for each coordinate $i$, we have
 \[0 \leq x^\frc_i \leq x^\frco_i \leq x^\itg_i \text{  or  } 0\leq x^\itg_i \leq x^\frco_i \leq x^\frc_i,\]
 depending on whether $x^\frc_i \leq x^\itg_i$ or $x^\itg_i \leq x^\frc_i$. Thus $x^\frco \in \sol^\R(P)$. This contradicts the optimality of $x^\frc$ since
 \[c^\trans x^\frco = c^\trans (x^\frc) + c^\trans(x^\itg - x^\itgo) < c^\trans x^\frc.\]
\end{proof}
\noindent
Despite being linked to existing notions of proximity by Lemma \ref{lem:proximity-optimal}, our interpretation of proximity will be central to the geometric decomposition approach we will take to prove our results. Our main idea will be to re-express the polyhedron associated to \eqref{eq:ilp-eq-form} as the intersection of several, simpler polyhedra. However, a optimal fractional solution to \eqref{eq:ilp-eq-form} does not necessarily correspond to a optimal fractional solution for each of these simpler polyhedra Our new notion of proximity overcomes this issue and allows for conceptually simple and robust arguments.
\subsection{Proximity bounds for $(r,s)$ stochastic matrices}
Key to our improved proximity bound is the following variant of a rearrangement lemma due to Klein. 
\begin{lemma}\label{lem:medium}
Let $T_1,\dots,T_k$ be nonempty multisets over $\Z^d_{\ge 0}$ so that for all $u \in T_i$, $\|u\|_{\infty} \leq \Delta$. Suppose there is $b \in \Z_{\geq 0}^d$ and $\delta \in \N \setminus\{0\}$ so that
	\[\Big\|\sum_{u\in T_i}u-b\Big\|_\infty < \delta\qquad \text{for all } i\in[k].\]
There is some function $f(\cdot, \cdot)$, only depending on $d$ and $\Delta$ but independent of $k$, so that if $\|b\|_{\infty} > \delta f(d,\Delta)$, there exists $c \in \Z_{\geq 0}^d$ with $c \leq b$ (component-wise) and submultisets $S_i \subseteq T_i$ such that
\[\sum_{u\in S_i}u=c \quad\text{for all }i\in [k] \quad \text{ and } \quad \|c\|_{\infty} \leq f(d,\Delta).\]
The function $f(d,\Delta)$ is bounded above by $\Oh(2^{(d\Delta)^{\Oh(d)}}).$
\end{lemma}
\noindent
Klein's original lemma only applied to the setting when the multisets add up to $b$ exactly, this is captured in the above when setting $\delta = 1$. This exact version was then used by Klein to bound the length of Graver basis elements. In our setting, we will decompose the difference between the optimal fractional solution and the optimal integral solution into Graver basis elements \emph{plus} some small error term. This slack-version of Klein's lemma above is tailored to handle this error incurred and is key for our argument. \\
\noindent
For the remainder of the section, we introduce some notation. Let $A$ a $(r,s)$-stochastic matrix corresponding to the (I)LP~\eqref{eq:ilp-eq-form}. Partition $x \in \R^m$ into $x = (x_0,x_1,\ldots,x_t)\in \R^{r + ts}$ so that $x_0\in \R^r$ corresponds to the columns of matrices $A_1,\ldots,A_t$, while $x_i\in \R^s$ corresponds to the columns of $B_i$, for each $i\in [t]$. Define $\pi_i$ so that $\pi_i(x) = x_i$ for all $i$. Partition $c$ into $c_0,c_1,\ldots,c_t$ in the same fashion, and partition $b$ into $b_1,\ldots,b_t$ so that each $b_i$ corresponds to the rows of $A_i$ and $B_i$.
We can now reformulate the Linear Program as follows:
\begin{align*}
	\min \sum_{i=0}^t c_i^\trans x_i &\\
	A_ix_0+B_ix_i = b_i & \qquad \textrm{for all }i\in \{1,\ldots,t\},\\
	x \geq 0.
\end{align*}
For every $i \in [t]$, we define the following polyhedron:
\begin{equation}\label{polyhedron:P_i}
	P_i:=\{x \in \R^{r+st}_{\geq 0} \,\mid\, A_i x_0 + B_i x_i = b_i, \quad x_j = 0 \quad \forall j \in [t]\setminus \{i\}\}.
\end{equation}
For all $i \in [t]$, define the projection $\Pi_i: \R^{r+st} \rightarrow \R^{r+st}$ so that $\Pi_i (x_0, x_1, \cdots, x_t)^\trans = \\
(x_0, 0, \cdots, 0, x_i, 0, \cdots)^\trans$. In words, $\Pi_i$ leaves $x_0$ and $x_i$ unchanged and sets all other components to $0$. The above reformulation of the Linear Program now corresponds to
\begin{alignat}{1}\label{reform:LP}
\begin{pmatrix}	x_0 \\ x_1 \\ \vdots\\ x_t
\end{pmatrix}\in \sol^\R(P)\quad\quad \textrm{if and only if}\quad\quad \Pi_i \begin{pmatrix}x_0 \\ x_1 \\ \vdots\\ x_t \end{pmatrix}\in \sol^\R(P_i)\quad\textrm{for all }i\in [t].
\end{alignat}
\noindent
This shows that the polyhedron $\sol^\R(P)$ can be seen as the intersection of the lifts of the polyhedra $P_i$. Each polyhedron $P_i$ is much simpler to describe (it is essentially $r + s$ dimensional) and their respective lifts only intersect in a single component $x_0$. This geometric decomposition of $\sol^\R(P)$ into simpler polyhedra leads to the following theorem relating the proximity of $P$ to the proximity of the $P_i$.

\begin{theorem}[Composition Theorem]\label{lem:proximity-uberlemma}
	Let $P=(x,A,b,c)$ a linear program in the form~\eqref{eq:ilp-eq-form} where $A$ is $(r,s)$-stochastic. Define
	$$
	\gamma\coloneqq \max_{1\leq i\leq t}\ g_\infty(A_i B_i)\qquad \textrm{and}\qquad
	\rho\coloneqq \max_{1\leq i\leq t}
	\ \proximity(P_i).$$
	The $P_i$ are the polyhedra defined in (\ref{polyhedron:P_i}) and $A_i B_i$ denotes the integral matrix where we concatenate the columns of $A_i$ and $B_i$ arising in the description of $P_i$. Then
	$$\proximity(P)\leq \rho \, (r\,\gamma\, f(r,\gamma) + 1).$$ 
\end{theorem}
\begin{proof}
	Let $x^\frc$ any fixed solution to $P$. Among all integral solutions with minimal $\ell_\infty$ distance to $x^\frc$, pick an integral solution $x^\itg$ minimizing $\|x^\frc - x^\itg\|_{1}$. 	
	To facilitate the proof, we will assume that $x^\itg = 0$ and $x^\frc \geq 0$. Formally, this can be achieved by tranlating $\sol^\R(P)$ by $-x^\itg$ and by identifying $+$ with $-$ if necessary. In particular, the integral points in the resulting polyhedron are elements of $\ker(A)$ and can be expressed as sum of Graver elements. We leave the details to the reader.\\
	Assume towards a contradiction that $\|x^\frc - x^\itg\|_{\infty} = \|x^\frc\|_{\infty} > \rho \, (r\,\gamma\, f(r,\gamma) + 1)$. We will now use our slack version of the Klein lemma to exhibit a non zero, integral point $x^\itgo \in P$ with $ 0 = x^\itg \lneq x^\itgo \leq x^\frc$. Since $\|x^\frc - x^\itgo\|_{\infty} \leq \|x^\frc - x^\itg\|_{\infty}$ but $\|x^\frc-x^\itgo\|_1 < \|x^\frc -x^\itg\|_{\infty} $, this will result in a contradiction.\\
	$\Pi_i(x^\frc), \Pi_i(0) \in P_i$ for all $i$. It follows that there are $x^\itgo_1, \cdots, x^\itgo_t \in \Z_{\geq 0}^m$ such that
	\begin{alignat}{1}\label{composition:close}
	\forall i \in [t]: \quad x^\itgo_i \in P_i, \quad 0 \leq x_i^\itgo \leq x^\frc \quad \text{ and } \quad \|\Pi_i(x^\frc)-x^\itgo_i\|_{\infty}  \leq \proximity(P_i)\leq \rho.
	\end{alignat}
	Each $x_i^\itgo \in \Z_{\geq 0}^m$ belongs to the kernel of the matrix $(A_i B_i)$ defining $P_i$ (we may leave out $0$ columns). It follows that the $x_i^\itgo$ can be decomposed into Graver basis elements of $\ell_{\infty}$ length bounded by $\gamma = \max_{1\leq i\leq t}\ g_\infty(A_i B_i)$. Specifically, there are multisets $T_1, \cdots, T_t$ consisting of respective Graver basis elements so that
	\begin{alignat}{1}\label{lem:composition_decomposition}
	\forall i\in [t]: \quad x_i^\itgo = \sum_{g \in T_i}g, \quad 0 \leq g \leq x_i^\itgo, \quad g \in P_i \quad \text{and} \quad \|g\|_{\infty} \leq \gamma.
	\end{alignat}
	From this decomposition, combined with $0 \leq x_i^\itgo \leq x^\frc$, we infer that
	\begin{alignat}{1}\label{lem:composition_lowerbound}
		\|\pi_0(x^\frc)\|_{\infty} \geq \frac{1}{r\gamma}\max_{1\leq i\leq t}\|\pi_i(x_i^{\itgo})\|_{\infty} \quad (> \rho \, f(r, \gamma))
	\end{alignat}
	Indeed, any Graver element in $g$ appearing in (\ref{lem:composition_decomposition}) with $\pi_0(g) = 0$ would verify $0 = x^\itg \leq g \leq x^\frc$ and, by (\ref{reform:LP}), would belong to $P$, contradicting the minimality of $\|x^\frc-x^\itg\|_1$. Thus, since all Graver elements are only supported on one component other than $x_0$, each Graver basis element needs to contribute $1$ to one of the $r$ columns of the zeroth component of $\pi_0(x_i^\itgo)$. Since $\pi_0(x_i^\itgo) \leq \pi_0(x^\frc)$, (\ref{lem:composition_lowerbound}) follows by averaging.
	We restrict (\ref{lem:composition_decomposition}) to the zeroth component and combine it with (\ref{composition:close}), see Figure \ref{illustration:proofcomposition}:
	\begin{alignat*}{1}
	\forall i\in [t]: \quad \|\sum_{g \in T_i}\pi_0(g) - \pi_0(x^\frc)\|_{\infty} \leq \rho, \quad \pi_0(g) \in \Z_{\geq 0}^r, \quad \|\pi_0(g)\|_{\infty} \leq \gamma.
	\end{alignat*}
	By Klein, $\forall i \in [t]$, there are non empty subsets $C_i \subseteq T_i$ and some $b \in \Z_{\geq 0}^r$ with $b \leq \pi_0(x^\frc)$ such that
	\begin{alignat*}{1}
		\forall i \in [t]: \quad \|\sum_{g \in C_i}\pi_0(g)\|_{\infty} = b \quad \text{ and } \quad \|b\|_{\infty} \leq  f(r,\gamma)
	\end{alignat*}
	Consider the following integral point:
	\begin{alignat*}{1}
		(x^\itgo)^{\trans} = \left(b, \sum_{g \in C_1}\pi_1(g), \sum_{g \in C_2}\pi_2(g), \cdots, \sum_{g \in C_t}\pi_t(g)\right).
	\end{alignat*}
Clearly, $\Pi_i(x^\itgo) \in P_i$ for all $i \in [t]$. Thus, by ($\ref{reform:LP})$, $x^\itgo \in P$ and, by positivity, $x^\itg \lneq x^\itgo \leq x^\frc$. This is a contradiction and we deduce $\|x^\frc - x^\itg\|_{\infty} \leq \rho \, (r\,\gamma\, f(r,\gamma) + 1)$
	
%	 Formally, this can be achieved by translating $\sol^\R(P), x^\frc$ and $x^\itg$ by $-x^\itg$. This preserves the matrices defining the polyhedra $\sol^\R(P)$ and $P_i$ for all $i \in [t]$ and preserves distances. The translation has the effect of replacing the positivity condition $x \geq 0$ by $x \geq -x^\frc$ for $\sol^\R(P)$ and the $P_i$ (for the non-zero coordinates).  Finally, up to flipping coordinates, we may assume that $0 = x^\itg \leq x^\frc$. 
	
\begin{figure}
	
	\centering
	\begin{tikzpicture}

		\draw[->] (-0.3,0)--(6.5,0) node[right]{};
		\draw[->] (0,-0.3)--(0,3.7) node[above]{};
		\node[fill, draw, circle, inner sep=1pt, black, label={[font = \small, yshift = -0.1cm]90:$\pi_0(x^{\frc})$}] at (5.5,3.3) {};
		\node [draw, dashed, shape=rectangle, minimum width=1.5cm, minimum height=1.5cm, anchor=center] at (5.5,3.3) {}; %draws the rectangle around x star
		\node[fill, draw, circle, inner sep=1pt, black, label={[font = \small]250:$ \pi_0(x^{\itg})$}] at (0,0) {};
		\draw[black] (0,0) rectangle (5.5, 3.3);
		%1st sequence, contains (2.5,1.8) see vectors with stars.
		\draw[->, gray] (0,0) -- (1, 0.2); %+(1,0.2)
		\draw[->, gray] (1, 0.2) -- (2, 0.7);%+(1, 0.5)
		\draw[->, gray] (2,0.7) -- (3, 1.5);%+(1, 0.8)**
		\draw[->, gray] (3,1.5) -- (3.9, 1.5);%+(0.8, 0)**
		\draw[->, gray] (3.9,1.5) -- (4.5, 1.7);%+(0.6, 0.2)**
		\draw[->, gray] (4.5, 1.7) -- (5.9, 1.8);%+(1.4, 0.2)
		\draw[->, gray] (5.9,1.8) -- (6.0, 2.6);%+(0.1, 0.8)**
		\node[fill, draw, circle, inner sep=1pt, black, label={[font = \tiny, yshift = -0.2cm, xshift = -0.1cm]0:$ \pi_0(x^{\itgo}_1)$}] at (6.0, 2.6) {};
		%2nd sequence, contains (2.5, 1.8)
		\draw[->, gray] (0,0) -- (0.2, 0.9); %+(0.2,0.9)**
		\draw[->, gray] (0.2, 0.9) -- (0.6, 1.7);%+(0.4, 0.8)**
		\draw[->, gray] (0.6, 1.7) -- (1.8, 1.9);%+(1.2, 0.1)**
		\draw[->, gray] (1.8, 1.9) -- (2.8, 2.3);%+(1, 0.4)
		\draw[->, gray] (2.8, 2.3) -- (3.5, 2.3);%+(0.7, 0)**
		\draw[->, gray] (3.5, 2.3) -- (4.5, 2.5);%+(1, 0.2)
		\draw[->, gray] (4.5, 2.5) -- (5, 2.9);%+(0.5, 0.4)
		\node[fill, draw, circle, inner sep=1pt, black, label={[font = \tiny, xshift = 0.05cm]180:$ \pi_0(x^{\itgo}_2)$}] at (5, 2.9) {};
		%3rd sequence, contains (2.5, 1.8)
		\draw[->, gray] (0,0) -- (0.7, 0.8); %+(0.7,0.8)**
		\draw[->, gray] (0.7, 0.8) -- (1.7, 0.9);%+(1.2, 0.2)
		\draw[->, gray] (1.7, 0.9) -- (2.3, 1.2);%+(0.6, 0.3)**
		\draw[->, gray] (2.3, 1.2) -- (3.4, 1.2);%+(1.2, 0.0)
		\draw[->, gray] (3.4, 1.2) -- (3.6, 1.8);%+(0.2, 0.6)
		\draw[->, gray] (3.6, 1.8) -- (3.9, 1.9);%+(0.3, 0.1)**
		\draw[->, gray] (3.9, 1.9) -- (4.0, 3.2);%+(0.1, 1.3)
		\draw[->, gray] (4.0, 3.2) -- (4.9, 3.8);%+(0.9, 0.6)**
		\draw[->, gray] (4.9, 3.8) -- (5.7, 4.0);%+(0.8, 0.2)
		\node[fill, draw, circle, inner sep=1pt, black, label={[font = \tiny, yshift = -0.07cm]90:$ \pi_0(x^{\itgo}_3)$}] at (5.7, 4.0) {};
	\end{tikzpicture}
	\caption{Different sets of projected vectors, summing to projections of integer vectors $\pi_0(x^{\itgo}_1), \pi_0(x^{\itgo}_2), \pi_0(x^{\itgo}_3)$ close to $\pi_0(x^\frc)$. THIS NEEDS CORRECTING $\pi_0(x_i^\itgo) \leq \pi_0(x^\frc)$!}	
	\label{illustration:proofcomposition}
\end{figure}
	
	
	
	
	
	
	
\end{proof}



\subsection{Proximity bounds for matrices with bounded tree-width}
\subsection{Improving the Klein lemma}	


Now we look at the special case of linear programs with one row. This will be used as the base case in our proofs of proximity bounds both for programs with bounded primal treedepth, and for $(r,s)$-stochastic programs.

\begin{lemma}\label{lem:proximity-one-row}
 Let $P=(x,a^\trans,b,c)$ be a linear program in the form \eqref{eq:ilp-eq-form}, where $a\in \mathbb{Z}^m$. Then 
 $$\proximity(P)\le (2\|a\|_{\infty}+1)m$$
\end{lemma}


